MVBench: A Comprehensive Multi-modal Video Understanding Benchmark

With the rapid development of Multi-modal Large Language Models (MLLMs), a number of diagnostic benchmarks have recently emerged to evaluate the comprehension capabilities of these models. However, most benchmarks predominantly assess spatial understanding in the static image tasks, while overlooking temporal understanding in the dynamic video tasks. To alleviate this issue, we introduce a comprehensive Multi-modal Video understanding Benchmark, namely MVBench, which covers 20 challenging video tasks that cannot be effectively solved with a single frame. Specifically, we first introduce a novel static-to-dynamic method to define these temporal-related tasks. By transforming various static tasks into dynamic ones, we enable the systematic generation of video tasks that require a broad spectrum of temporal skills, ranging from perception to cognition. Then, guided by the task definition, we automatically convert public video annotations into multiple-choice QA to evaluate each task. On one hand, such a distinct paradigm allows us to build MVBench efficiently, without much manual intervention. On the other hand, it guarantees evaluation fairness with ground-truth video annotations, avoiding the biased scoring of LLMs. Moreover, we further develop a robust video MLLM baseline, i.e., VideoChat2, by progressive multi-modal training with diverse instruction-tuning data. The extensive results on our MVBench reveal that, the existing MLLMs are far from satisfactory in temporal understanding, while our VideoChat2 largely surpasses these leading models by over 15% on MVBench. All models and data are available at https://github.com/OpenGVLab/Ask-Anything.

==> tables/mvpbench2.tex <==
\begin{table*}[tp]
    \centering
    \setlength\tabcolsep{1pt}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        \Xhline{1.0pt}
        \textbf{Model} & \textbf{LLM} & \textbf{Avg} & \textbf{AS} & \textbf{AP} & \textbf{AA} & \textbf{FA} & \textbf{UA} & \textbf{OE} & \textbf{OI} & \textbf{OS} & \textbf{MD} & \textbf{AL} & \textbf{ST} & \textbf{AC} & \textbf{MC} & \textbf{MA} & \textbf{SC} & \textbf{FP} & \textbf{CO} & \textbf{EN} & \textbf{ER} & \textbf{CI} \\
        \Xhline{1.0pt}
        Random & - & \cellcolor{gray!20}{27.3} & 25.0 & 25.0 & 33.3 & 25.0 & 25.0 & 33.3 & 25.0 & 33.3 & 25.0 & 25.0 & 25.0 & 33.3 & 25.0 & 33.3 & 33.3 & 25.0 & 33.3 & 25.0 & 20.0 & 30.9 \\
        \Xhline{0.8pt}
        \multicolumn{23}{l}{\gray{\textit{GPT-4V take \textbf{16} frames as input, and the resolution is \textbf{512$\times$512}, while others use small resolution of \textbf{224$\times$224}.}}} \\
        GPT-4V~\cite{gpt4v} & GPT-4 & \cellcolor{gray!20}{49.5} & \textbf{80.0} & 40.0 & 30.0 & 50.0 & \textbf{60.0} & 60.0 & \textbf{90.0} & 40.0 & 20.0 & \textbf{60.0} & \textbf{100.0} & 40.0 & 20.0 & \textbf{50.0} & 40.0 & \textbf{70.0} & \textbf{50.0} & 20.0 & \textbf{60.0} & 10.0 \\
        \Xhline{0.8pt}
        \multicolumn{23}{l}{\gray{\textit{\textbf{Image MLLMs:} Following~\cite{instructblip}, all models take \textbf{4} frames as input, with the output embeddings concatenated before feeding into the LLM.}}} \\
        Otter-I~\cite{otter} & MPT-7B & \cellcolor{gray!20}{35.0} & 50.0 & 30.0 & 20.0 & 30.0 & 40.0 & 50.0 & 50.0 & 30.0 & 30.0 & 10.0 & 40.0 & 40.0 & 20.0 & 40.0 & 40.0 & 40.0 & 30.0 & 30.0 & 40.0 & 40.0 \\
        InstructBLIP~\cite{instructblip} & Vicuna-7B & \cellcolor{gray!20}{34.0} & 40.0 & 50.0 & 40.0 & 40.0 & 40.0 & 60.0 & 40.0 & 10.0 & 20.0 & 20.0 & 70.0 & 30.0 & 20.0 & 30.0 & 50.0 & 40.0 & 20.0 & 20.0 & 30.0 & 10.0 \\
        LLaVA~\cite{llava} & Vicuna-7B & \cellcolor{gray!20}{34.5} & 40.0 & 30.0 & 20.0 & 30.0 & \textbf{60.0} & 50.0 & 30.0 & 20.0 & 30.0 & 30.0 & 40.0 & 20.0 & \textbf{40.0} & 30.0 & 40.0 & 30.0 & 40.0 & 20.0 & 50.0 & 40.0 \\
        \Xhline{0.8pt}
        \multicolumn{23}{l}{\gray{\textit{\textbf{Video MLLMs:} All models take \textbf{16} frames as input, with the exception of VideoChatGPT, which uses \textbf{100} frames.}}} \\
        VideoChatGPT~\cite{videochatgpt} & Vicuna-7B & \cellcolor{gray!20}{32.5} & 30.0 & 30.0 & 50.0 & 30.0 & 40.0 & 70.0 & 20.0 & \textbf{50.0} & 10.0 & 20.0 & 10.0 & 30.0 & 10.0 & 30.0 & \textbf{70.0} & 20.0 & \textbf{50.0} & 10.0 & 50.0 & 20.0 \\
        VideoLLaMA~\cite{videollama} & Vicuna-7B & \cellcolor{gray!20}{34.0} & 30.0 & 20.0 & 50.0 & 40.0 & 20.0 & 50.0 & 40.0 & 0.0 & 30.0 & 10.0 & 70.0 & 40.0 & 30.0 & 30.0 & 50.0 & 30.0 & \textbf{50.0} & 50.0 & 40.0 & 0.0 \\
        VideoChat~\cite{videochat} & Vicuna-7B & \cellcolor{gray!20}{36.5} & 50.0 & 10.0 & 50.0 & 20.0 & 50.0 & 60.0 & 70.0 & 40.0 & \textbf{40.0} & 40.0 & 50.0 & 30.0 & 20.0 & 40.0 & 50.0 & 20.0 & 30.0 & 10.0 & 50.0 & 0.0 \\
        \hline
        \textbf{\ModelName$_\mathbf{text}$} & Vicuna-7B & \cellcolor{gray!20}{35.0} & 40.0 & 40.0 & 30.0 & 30.0 & 30.0 & 40.0 & 20.0 & \textbf{50.0} & 20.0 & 30.0 & 60.0 & \textbf{60.0} & 30.0 & 20.0 & 60.0 & 20.0 & \textbf{50.0} & 30.0 & 30.0 & 10.0 \\
        \textbf{\ModelName} & Vicuna-7B & \cellcolor{gray!20}{\textbf{56.5}} & 60.0 & \textbf{60.0} & \textbf{90.0} & \textbf{60.0} & \textbf{60.0} & \textbf{70.0} & 80.0 & 30.0 & 20.0 & 40.0 & \textbf{100.0} & 40.0 & \textbf{40.0} & 40.0 & 60.0 & 50.0 & 40.0 & \textbf{60.0} & \textbf{60.0} & \textbf{70.0} \\
        \Xhline{1.0pt}
        \end{tabular}
    }
    \vspace{-0.3cm}
    \caption{
    \textbf{Evaluations results on \BenchName\ subset.}
    We randomly sample 10 multiple-choice QAs for each task due to time constraints. 
    The results on full MVBench can be found at \url{https://huggingface.co/spaces/OpenGVLab/MVBench_Leaderboard}.}
    \label{tab:mvpbench2}
    \vspace{-0.5cm}
\end{table*}
